Scheduling Dags under Uncertainty

This paper introduces a parallel scheduling problem where a directed acyclic graph modeling $t$ tasks and their dependencies needs to be executed on $n$ unreliable workers. Worker $i$ executes task $j$ correctly with probability $p_{i,j}$. The goal is to find a regimen $\Sigma$, that dictates how workers get assigned to tasks (possibly in parallel and redundantly) throughout execution, so as to minimize the expected completion time. This fundamental parallel scheduling problem arises in grid computing and project management fields, and has several applications. We show a polynomial time algorithm for the problem restricted to the case when dag width is at most a constant and the number of workers is also at most a constant. These two restrictions may appear to be too severe. However, they are fundamentally required. Specifically, we demonstrate that the problem is NP-hard with constant number of workers when dag width can grow, and is also NP-hard with constant dag width when the number of workers can grow. When both dag width and the number of workers are unconstrained, then the problem is inapproximable within factor less than 5/4, unless P=NP.

==> preamble.tex <==
\def \eqdef {\stackrel{\mbox{{\tiny def}}}{=}}
\newcommand{\comment}[1]{}
\renewcommand{\Box}{\nopagebreak\mbox{}\hfill{\rule{2mm}{2mm}}\medskip}
%\newcommand{\qed}{\nopagebreak\mbox{}\hfill{\rule{2mm}{2mm}}\medskip}

%Full-size script letters
\renewcommand{\a}{\mbox{$\cal A$}}
\renewcommand{\b}{\mbox{$\cal B$}}
\renewcommand{\c}{\mbox{$\cal C$}}
\renewcommand{\d}{\mbox{$\cal D$}}
\newcommand{\e}{\mbox{$\cal E$}}
\newcommand{\f}{\mbox{$\cal F$}}
\newcommand{\g}{\mbox{$\cal G$}}
\newcommand{\h}{\mbox{$\cal H$}}
\renewcommand{\i}{\mbox{$\cal I$}}
\renewcommand{\j}{\mbox{$\cal J$}}
\renewcommand{\k}{\mbox{$\cal K$}}
\renewcommand{\l}{\mbox{$\cal L$}}
\newcommand{\m}{\mbox{$\cal M$}}
\newcommand{\n}{\mbox{$\cal N$}}
\renewcommand{\o}{\mbox{$\cal O$}}
\newcommand{\p}{\mbox{$\cal P$}}
\newcommand{\q}{\mbox{$\cal Q$}}
\renewcommand{\r}{\mbox{$\cal R$}}
\newcommand{\s}{\mbox{$\cal S$}}
\renewcommand{\t}{\mbox{$\cal T$}}
\renewcommand{\u}{\mbox{$\cal U$}}
\newcommand{\w}{\mbox{$\cal W$}}
\newcommand{\x}{\mbox{$\cal X$}}
\newcommand{\y}{\mbox{$\cal Y$}}
\newcommand{\z}{\mbox{$\cal Z$}}

%subscript-size script letters
\newcommand{\fa}{\mbox{{\scriptsize $\cal A$}}}
\newcommand{\fb}{\mbox{{\scriptsize $\cal B$}}}
\newcommand{\fc}{\mbox{{\scriptsize $\cal C$}}}
\newcommand{\fd}{\mbox{{\scriptsize $\cal D$}}}
\newcommand{\fe}{\mbox{{\scriptsize $\cal E$}}}
\newcommand{\ff}{\mbox{{\scriptsize $\cal F$}}}
\newcommand{\fg}{\mbox{{\scriptsize $\cal G$}}}
\newcommand{\fh}{\mbox{{\scriptsize $\cal H$}}}
\newcommand{\fii}{\mbox{{\scriptsize $\cal I$}}}
\newcommand{\fj}{\mbox{{\scriptsize $\cal J$}}}
\newcommand{\fk}{\mbox{{\scriptsize $\cal K$}}}
\newcommand{\fl}{\mbox{{\scriptsize $\cal L$}}}
\newcommand{\fm}{\mbox{{\scriptsize $\cal M$}}}
\newcommand{\fn}{\mbox{{\scriptsize $\cal N$}}}
\newcommand{\fo}{\mbox{{\scriptsize $\cal O$}}}
\newcommand{\fp}{\mbox{{\scriptsize $\cal P$}}}
\newcommand{\fq}{\mbox{{\scriptsize $\cal Q$}}}
\newcommand{\fr}{\mbox{{\scriptsize $\cal R$}}}
\newcommand{\fs}{\mbox{{\scriptsize $\cal S$}}}
\newcommand{\ft}{\mbox{{\scriptsize $\cal T$}}}
\newcommand{\fu}{\mbox{{\scriptsize $\cal U$}}}
\newcommand{\fv}{\mbox{{\scriptsize $\cal V$}}}
\newcommand{\fw}{\mbox{{\scriptsize $\cal W$}}}
\newcommand{\fx}{\mbox{{\scriptsize $\cal X$}}}
\newcommand{\fy}{\mbox{{\scriptsize $\cal Y$}}}
\newcommand{\fz}{\mbox{{\scriptsize $\cal Z$}}}

\newcommand{\E}{\mbox{\sf E}}
\newcommand{\N}{\mbox{\sf N}}
\newcommand{\G}{\mbox{\bf G}}
\newcommand{\HH}{\mbox{\bf H}}

%CLIQUE-RELATED GRAPHS
% n-node complete graph
\newcommand{\kn}{\mbox{$\k_n$}}
\newcommand{\fkn}{\mbox{{\scriptsize $\k_n$}}}
% n-by-n complete bipartite graph
\newcommand{\knn}{\mbox{$\k_{n,n}$}}
\newcommand{\fknn}{\mbox{{\scriptsize $\k_{n,n}$}}}
%m x n mesh of cliques
\newcommand{\moc}{\mbox{${\cal MC}_{m,n}$}}
\newcommand{\fmoc}{\mbox{{\scriptsize ${\cal MC}_{m,n}$}}}
%n x n mesh of cliques
\newcommand{\mocs}{\mbox{${\cal MC}_{n,n}$}}
\newcommand{\fmocs}{\mbox{{\scriptsize ${\cal MC}_{n,n}$}}}

%PATH-LIKE GRAPHS
%length-n paths
%\newcommand{\path}{\mbox{$\p_n$}}
\newcommand{\fpath}{\mbox{{\scriptsize $\p_n$}}}
%length-n cycles
\newcommand{\cycle}{\mbox{$\c_n$}}
\newcommand{\fcycle}{\mbox{{\scriptsize $\c_n$}}}

%TREE-RELATED GRAPHS
% height-h complete b-ary tree
\newcommand{\treegen}{\mbox{$\t_h(b)$}}
\newcommand{\ftreegen}{\mbox{{\scriptsize $\t_h(b)$}}}
% height-h complete binary tree
\newcommand{\tree}{\mbox{$\t_h$}}
\newcommand{\ftree}{\mbox{{\scriptsize $\t_h$}}}
% height-h complete ternary tree
\newcommand{\treet}{\mbox{$\t_h(3)$}}
\newcommand{\ftreet}{\mbox{{\scriptsize $\t_h(3)$}}}
% height-h X-tree
\newcommand{\xtree}{\mbox{$\x_h$}}
\newcommand{\fxtree}{\mbox{{\scriptsize $\x_h$}}}

%MESH-LIKE GRAPHS
%side-n d-dimensional toroidal mesh
\newcommand{\torusgen}{\mbox{$\widetilde{\m}_{n,n}(d)$}}
\newcommand{\ftorusgen}{\mbox{{\scriptsize $\widetilde{\m}_{n,n}(d)$}}}
%side-n d-dimensional mesh
\newcommand{\meshgen}{\mbox{$\m_n(d)$}}
\newcommand{\fmeshgen}{\mbox{{\scriptsize $\m_n(d)$}}}
%m x n 2-dimensional mesh
\newcommand{\mesh}{\mbox{$\m_{m,n}$}}
\newcommand{\fmesh}{\mbox{{\scriptsize $\m_{m,n}$}}}
%side-n 2-dimensional mesh
\newcommand{\meshs}{\mbox{$\m_{n,n}$}}
\newcommand{\fmeshs}{\mbox{{\scriptsize $\m_{n,n}$}}}
%m x n 2-dimensional toroidal mesh
\newcommand{\torus}{\mbox{$\widetilde{\m}_{m,n}$}}
\newcommand{\ftorus}{\mbox{{\scriptsize $\widetilde{\m}_{m,n}$}}}
%side-n 2-dimensional toroidal mesh
\newcommand{\toruss}{\mbox{$\widetilde{\m}_{n,n}$}}
\newcommand{\ftoruss}{\mbox{{\scriptsize $\widetilde{\m}_{n,n}$}}}

%HYPERCUBE-RELATED GRAPHS
%base-b n-dimensional hypercube
\newcommand{\cubegen}{\mbox{$\q_n(b)$}}
\newcommand{\fcubegen}{\mbox{{\scriptsize $\q_n(b)$}}}
%base-2 (boolean) n-dimensional hypercube
\newcommand{\cube}{\mbox{$\q_n$}}
\newcommand{\fcube}{\mbox{{\scriptsize $\q_n$}}}

%BUTTERFLY-LIKE GRAPHS
%base-2, order-n butterfly
\newcommand{\but}{\mbox{$\b_n$}}
\newcommand{\fbut}{\mbox{{\scriptsize $\b_n$}}}
%base-b, order-n butterfly
\newcommand{\butgen}{\mbox{$\b_n(b)$}}
\newcommand{\fbutgen}{\mbox{{\scriptsize $\b_n(b)$}}}
%base-2, order-n FFT graph
\newcommand{\fft}{\mbox{$\f_n$}}
\newcommand{\ffft}{\mbox{{\scriptsize $\f_n$}}}
%base-2, order-n cube-connected cycles graph
\newcommand{\ccc}{\mbox{${\c\c\c}_n$}}
\newcommand{\fccc}{\mbox{{\scriptsize ${\c\c\c}_n$}}}
%base-b, order-n cube-connected cycles graph
\newcommand{\cccgen}{\mbox{${\c\c\c}_n(b)$}}
\newcommand{\fcccgen}{\mbox{{\scriptsize ${\c\c\c}_n(b)$}}}

%SHUFFLE-LIKE GRAPHS
%base-b, order-n de Bruijn graph
\newcommand{\dbgen}{\mbox{$\d_n(b)$}}
\newcommand{\fdbgen}{\mbox{{\scriptsize $\d_n(b)$}}}
%base-2, order-n de Bruijn graph
\newcommand{\db}{\mbox{$\d_n$}}
\newcommand{\fdb}{\mbox{{\scriptsize $\d_n$}}}
%base-2, order-n shuffle-exchange
\newcommand{\se}{\mbox{$\s_n$}}
\newcommand{\fse}{\mbox{{\scriptsize $\s_n$}}}
%base-b, order-n shuffle-exchange
\newcommand{\segen}{\mbox{$\f_n(b)$}}
\newcommand{\fsegen}{\mbox{{\scriptsize $\s_n(b)$}}}

\comment{***************
\setcounter{appl}{0}
\setcounter{corol}{0}
\setcounter{fact}{0}
\setcounter{need}{0}
\setcounter{prop}{0}
\setcounter{theorem}{0}
****************}



% ............................................. Added by Vittorio
%-----------------------------------------------------------------------
%                        FIGURES ENVIRONMENT
%-----------------------------------------------------------------------
%
% ................... max width for the boix contatining a figure
\newlength{\figtextwidth}
\setlength{\figtextwidth}{\textwidth}
\addtolength{\figtextwidth}{-12pt}

%.................... max width for the figure inside the box
\newlength{\figmaxwidth}
\setlength{\figmaxwidth}{\textwidth}
\addtolength{\figmaxwidth}{-70pt}

%.................... max height for the figure inside the box
\newlength{\figmaxheight}
\setlength{\figmaxheight}{\textheight}
\addtolength{\figmaxheight}{-2truecm}


%.......................... current value for width of the gifure
%inside
% This is the value used by the macro. It can be modified for
% particularly small figures but it should be reset immediately after
% the
% figure to the defualt value \figmaxwidth.
\newlength{\figwidth}
\setlength{\figwidth}{\figmaxwidth}

%----------------------------------------- MYFIGUREPS environment
% USAGE: \myfigureps{position}{filename}{caption}{label}
\newcommand{\myfigureps}[4]{
\begin{figure}[#1]
\begin{tabular}{|p{\figtextwidth}|}  \hline\\
\centerline{\psfig{figure=#2.eps,width=\figwidth}}
\\ \hline \end{tabular}
\refstepcounter{figure}\label{#4}
%\vspace{-1em} the quote environment adds too much vspace
%\centerline{
\begin{quote}\noindent\sc\small Figure \thefigure: \small #3
\hspace*{\fill}
%}
\setlength{\baselineskip}{5pt}
\end{quote}
\vspace{-1em} %the quote environment adds too much vspace
\normalsize\rm\vspace{-1ex}% do not waste vertical space!
\end{figure}
}


%----------------------------------------- MYFIGURE environment
% USAGE: \myfigure{position}{body_of_figure}{width}{caption}{label}
%        use \figmaxwidth for width if you want the max width
\newcommand{\myfigure}[5]{
\begin{figure}[#1]
\begin{center}
\begin{tabular}{|p{#3}|}  \hline\\ \vspace{-1truecm}#2 \\ \hline
\end{tabular}
\end{center}
\refstepcounter{figure}\label{#5}
\vspace{-1em} %...............the quote environment adds too much
	      %vspace
\begin{quote}\noindent\sc\small Figure \thefigure: \it\small #4
\hspace*{\fill}
\setlength{\baselineskip}{5pt}
\end{quote}
\vspace{-1em} %...............the quote environment adds too much
	      %vspace
\normalsize\rm\vspace{-1ex}% do not waste vertical space!
\end{figure}
}

